Answerability Fields: Answerable Location Estimation via Diffusion Models

In an era characterized by advancements in artificial intelligence and robotics, enabling machines to interact with and understand their environment is a critical research endeavor. In this paper, we propose Answerability Fields, a novel approach to predicting answerability within complex indoor environments. Leveraging a 3D question answering dataset, we construct a comprehensive Answerability Fields dataset, encompassing diverse scenes and questions from ScanNet. Using a diffusion model, we successfully infer and evaluate these Answerability Fields, demonstrating the importance of objects and their locations in answering questions within a scene. Our results showcase the efficacy of Answerability Fields in guiding scene-understanding tasks, laying the foundation for their application in enhancing interactions between intelligent agents and their environments.

==> fig/moduleTest.tex <==
\begin{figure*}
\begin{center}
\includegraphics[keepaspectratio, scale=0.5]{fig/ModuleTest.pdf}
\end{center}
\vspace{-0.4cm}
\caption{
%Supplementing the point cloud on the floor for increasing the navigable area.
%Compare the best pose between best view and answerability score.
We propose answerability fields to make agent efficiently learn navigation path. We compute the score of answerability to the questions in each location by using strong Visual Question Answering (VQA) model called OFA.}
\label{fig:moduletest}
\vspace{-0.3cm}
\end{figure*}

==> tab/datasplit.tex <==
\renewcommand{\arraystretch}{1.0}
\begin{table}
\begin{center}
	\small\begin{tabular}{lcccc}
        \toprule
Split        &\# 3D scenes & \# Questions & \# Unique question.\\
\midrule
Train           & 494 & 32,255 & 25,628 \\
Val             & 68  & 4,260  &  3,972 \\
Test            & 57 & 4,111  &  3,794 \\
\midrule
Total           & 619 & 40,626 & 31,741\\
\bottomrule
	\end{tabular}
	\vspace{0.2cm}
    \caption{
        AnswerabilityFields dataset statistics.
    }
    \label{table:datasplit}
\end{center}
%\vspace{-4mm}
%\vspace{0.2cm}
\end{table}
